Adaptive Gaussian Processes on Graphs via Spectral Graph Wavelets

Graph-based models require aggregating information in the graph from neighbourhoods of different sizes. In particular, when the data exhibit varying levels of smoothness on the graph, a multi-scale approach is required to capture the relevant information. In this work, we propose a Gaussian process model using spectral graph wavelets, which can naturally aggregate neighbourhood information at different scales. Through maximum likelihood optimisation of the model hyperparameters, the wavelets automatically adapt to the different frequencies in the data, and as a result our model goes beyond capturing low frequency information. We achieve scalability to larger graphs by using a spectrum-adaptive polynomial approximation of the filter function, which is designed to yield a low approximation error in dense areas of the graph spectrum. Synthetic and real-world experiments demonstrate the ability of our model to infer scales accurately and produce competitive performances against state-of-the-art models in graph-based learning tasks.

==> data_efficiency_plot.tex <==







\begin{figure*}
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \begin{tikzpicture}
    \pgfkeys{/pgfplots/MyAxisStyle/.style={width=1.1\linewidth, height=0.86\linewidth}}
    \pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.4ex}}
    \pgfplotsset{every y tick label/.append style={font=\tiny, xshift=0.4ex}}
    \pgfplotsset{xlabel style={font=\tiny, yshift=0.35cm}}
    \pgfplotsset{ylabel style={font=\tiny, yshift=-0.7cm}}
    \begin{axis}[MyAxisStyle, ylabel=accuracy, xlabel=percentage of original training nodes, xmin=0.00, xmax=1.1, ymin=0.0, ymax=100.0, legend style={font=\tiny, draw=none, fill=none, at={(-0.04,1.15)}, anchor=west}, legend columns=5, name=plot11]
    
    \addlegendentry{WGGP}
    \addplot+[highlightGreen, mark options={highlightGreen!70}, line width=0.5pt] table[x=fraction, y=wggp, col sep=comma] {data_efficiency_cora.dat};
    \addlegendentry{GCN}
    \addplot+[highlightRed, mark options={highlightRed!70}, line width=0.5pt] table[x=fraction, y=gcn, col sep=comma] {data_efficiency_cora.dat};
    
    \end{axis}
    \end{tikzpicture}
    \caption{Cora}
    \label{fig:data_eff_cora} 
\end{subfigure}
%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \begin{tikzpicture}
    \pgfkeys{/pgfplots/MyAxisStyle/.style={width=1.1\linewidth, height=0.86\linewidth}}
    \pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.4ex}}
    \pgfplotsset{every y tick label/.append style={font=\tiny, xshift=0.4ex}}
    \pgfplotsset{xlabel style={font=\tiny, yshift=0.35cm}}
    \begin{axis}[MyAxisStyle, xlabel=percentage of original training nodes, xmin=0.00, xmax=1.1, ymin=0.0, ymax=100.0, legend style={font=\tiny, draw=none}, name=plot11]
    
    % \addlegendentry{WGGP}
    \addplot+[highlightGreen, mark options={highlightGreen!70}, line width=0.5pt] table[x=fraction, y=wggp, col sep=comma] {data_efficiency_citeseer.dat};
    % \addlegendentry{gcn}
    \addplot+[highlightRed, mark options={highlightRed!70}, line width=0.5pt] table[x=fraction, y=gcn, col sep=comma] {data_efficiency_citeseer.dat};
    
    \end{axis}
    \end{tikzpicture}
    \caption{Citeseer}
    \label{fig:data_eff_citeseer}
\end{subfigure}
%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \begin{tikzpicture}
    \pgfkeys{/pgfplots/MyAxisStyle/.style={width=1.1\linewidth, height=0.86\linewidth}}
    \pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.4ex}}
    \pgfplotsset{every y tick label/.append style={font=\tiny, xshift=0.4ex}}
    \pgfplotsset{xlabel style={font=\tiny, yshift=0.35cm}}
    \begin{axis}[MyAxisStyle, xlabel=percentage of original training nodes, xmin=0.00, xmax=1.1, ymin=0.0, ymax=100.0, legend style={font=\tiny, draw=none}, name=plot11]
    
    % \addlegendentry{WGGP}
    \addplot+[highlightGreen, mark options={highlightGreen!70}, line width=0.5pt] table[x=fraction, y=wggp, col sep=comma] {data_efficiency_pubmed.dat};
    % \addlegendentry{GCN}
    \addplot+[highlightRed, mark options={highlightRed!70}, line width=0.5pt] table[x=fraction, y=gcn, col sep=comma] {data_efficiency_pubmed.dat};
    
    \end{axis}
    \end{tikzpicture}
    \caption{PubMed}
    \label{fig:data_eff_pubmed}
\end{subfigure}
\caption{Prediction accuracy for different fractions of the original training nodes available for the Cora, Citeseer, and PubMed data sets. The results for $100\%$ of the training nodes corresponds to the results in Table~\ref{tab:results}.
}
\label{fig:data_efficiency}
\end{figure*}



==> overview.tex <==
    \begin{tikzpicture}
    \draw[scale=3, domain=0:2, smooth, variable=\x, highlightOrange, line width=1pt] plot ({\x}, {1.0 / (1.0 + 5 * \x)});
    \node[anchor=west, font=\small] at (0.1,3.0) {\textcolor{highlightOrange}{scaling filter $h^{1}_{\alpha}(\lambda)$}};
    \draw[scale=3, domain=0:2, smooth, variable=\x, highlightBlue, line width=1pt] plot ({\x}, {1.22664 * (2*\x)*(2*\x) * exp(-0.5 * (2*\x)*(2*\x))});
    \node[anchor=west, font=\small] at (2.9,2.2) {\textcolor{highlightBlue}{Wavelet filter $g^{1}_{\beta}(\lambda)$}};
    \draw[line width=0.5pt] (0.0,0.0) rectangle (6.0,4.5);
    \node[anchor=center] at (3.0, -0.5) {eigenvalues $\lambda$};
    \node[anchor=center, rotate=90] at (-0.4, 2.0) {filter values};
    
    % eigenvalues
    \node at (0.0, 0.0) {$\times$};
    \node at (0.15, 0.0) {$\times$};
    \node at (0.24, 0.0) {$\times$};
    \node at (0.32, 0.0) {$\times$};
    \node at (1.8, 0.0) {$\times$};
    \node at (2.0, 0.0) {$\times$};
    \node at (2.1, 0.0) {$\times$};
    \node at (2.28, 0.0) {$\times$};
    \node at (2.41, 0.0) {$\times$};
    \node at (2.57, 0.0) {$\times$};
    \node at (2.76, 0.0) {$\times$};
    
    %%%%%%%%% Cluster bottom centre %%%%%%%%% 
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n11) at (-5.0, 0.0) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n12) at (-5.5, 0.3) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n13) at (-4.6, 0.45) {};
    \draw (n11) -- (n12);
    \draw (n11) -- (n13);
    \draw (n12) -- (n13);
    
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n21) at (-7.0, 0.2) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n22) at (-7.2, 0.8) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n23) at (-6.3, 0.75) {};
    \draw (n21) -- (n22);
    \draw (n21) -- (n23);
    \draw (n22) -- (n23);
    \draw (n23) -- (n12);
    
    %%%%%%%%% Cluster top left %%%%%%%%%
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n31) at (-9.0, 2.2) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n32) at (-9.2, 2.8) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n33) at (-8.3, 2.75) {};
    \draw (n31) -- (n32);
    \draw (n31) -- (n33);
    \draw (n32) -- (n33);
    % \draw (n23) -- (n12);
    
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n41) at (-8.0, 3.2) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n42) at (-8.0, 4.0) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n43) at (-7.3, 3.75) {};
    \draw (n41) -- (n42);
    \draw (n41) -- (n43);
    \draw (n42) -- (n43);
    \draw (n41) -- (n33);
    
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n51) at (-7.7, 1.8) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n52) at (-8.0, 2.3) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n53) at (-7.05, 2.2) {};
    \draw (n51) -- (n52);
    \draw (n51) -- (n53);
    \draw (n52) -- (n53);
    \draw (n52) -- (n41);
    \draw (n52) -- (n31);
    \draw (n51) -- (n22);
    
    %%%%%%%%% Cluster top right %%%%%%%%% 
    \draw [highlightOrange, fill=highlightOrange!20] plot [smooth cycle] coordinates {(-4.4, 0.7) (-6.2, 3.1) (-2.8, 3.1)};
    
    \draw [highlightBlue, fill=highlightBlue!20] plot [smooth cycle] coordinates {(-3.65, 2.05) (-4.3, 3.2) (-3.1, 2.9)};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n61) at (-3.6, 2.3) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n62) at (-4.0, 3.0) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n63) at (-3.3, 2.75) {};
    \draw (n61) -- (n62);
    \draw (n61) -- (n63);
    \draw (n62) -- (n63);
    % \draw (n41) -- (n33);
    
    \draw [highlightBlue, fill=highlightBlue!20] plot [smooth cycle] coordinates {(-5.5, 1.75) (-5.6, 3.0) (-4.4, 2.65)};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n71) at (-5.4, 2.0) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n72) at (-5.4, 2.8) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n73) at (-4.8, 2.45) {};
    \draw (n71) -- (n72);
    \draw (n71) -- (n73);
    \draw (n72) -- (n73);
    \draw (n73) -- (n62);
    
    \draw [highlightBlue, fill=highlightBlue!20] plot [smooth cycle] coordinates {(-4.6, 1.0) (-4.6, 2.3) (-3.5, 1.7)};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n81) at (-4.4, 1.3) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n82) at (-4.5, 2.1) {};
    \node[circle, minimum width=0.3cm, line width=0.5pt, draw=black] (n83) at (-3.8, 1.8) {};
    \draw (n81) -- (n82);
    \draw (n81) -- (n83);
    \draw (n82) -- (n83);
    \draw (n82) -- (n73);
    \draw (n83) -- (n61);
    \draw (n81) -- (n13);
    
    
    \draw[<->, draw=highlightBlue, line width=0.5pt, dashed] (-3.8, 0.5) to[in=-160, out=-20] (-0.3, 0.5);
    \draw[<->, draw=highlightOrange, line width=0.5pt, dashed] (-3.8, 3.5) to[in=160, out=20] (-0.3, 3.5);
    
    \end{tikzpicture}
